Discourse-Based Objectives for Fast Unsupervised Sentence Representation Learning

This work presents a novel objective function for the unsupervised training of neural network sentence encoders. It exploits signals from paragraph-level discourse coherence to train these models to understand text. Our objective is purely discriminative, allowing us to train models many times faster than was possible under prior methods, and it yields models which perform well in extrinsic evaluations.

==> snli.tex <==
\paragraph{Sentence Pair Classification} \todo{If we're short on space, we can include SNLI in the main comparisons table. That'd mean nixing the baselines, though.} We also use the Stanford Natural Language Inference corpus \citep[SNLI;][]{DBLP:conf/emnlp/BowmanAPM15} as a reference dataset for semi-supervised learning. Here, we follow the approach of \citet{DBLP:journals/corr/VendrovKFU15}, training our sentence encoder in an unsupervised setting and using the large SNLI training set only to train an MLP to compute labels over pairs of sentence encodings. Looking at the results (Table~\ref{tab:snli}), it seems that we mostly capture syntax-type features, but adding simple pre-trained word embeddings brings us to the level of specific-purpose trained systems, a little worse than Skip Thought.

\todo{Should we comment on the mismatch in training accuracy between DiscSent and Skip Thought on SNLI?}


\begin{table}[h!]
\begin{centering}
\begin{tabular}{l c c }
\toprule
\bf Model                 & \bf Train & \bf Test \\
\toprule
Unlexicalized feats$^1$ & 49.4 & 50.4  \\ 
~+ Lexicalized feats$^1$      & 99.7 & 78.2  \\ 
300D LSTM$^2$           & 83.9 & 80.6  \\
300D NSE encoder$^{3}$  & 86.2 & \textbf{84.6}  \\
\midrule
1024D Skip Thought GRU$^{4}$        & 98.8 & 81.4  \\ 
DiscSent biGRU          & 64.8 & 65.0  \\
Embed only              & ? & ?  \\ 
DiscSent+embed          & 82.0 & 81.3  \\
\bottomrule
\end{tabular}
\caption{SNLI results using sentence encoders trained on both SNLI$^{1,2,3}$ and unlabeled data.$^4$ \todo{Include dimension of DiscSent. We can also cut the first two baselines if we need space.} References: $^1$\citet{DBLP:conf/emnlp/BowmanAPM15} $^2$\citet{bowman-EtAl:2016:P16-1} $^{3}$\citet{DBLP:journals/corr/MunkhdalaiY16}  $^{4}$\citet{DBLP:journals/corr/VendrovKFU15}}
\label{tab:snli}
\end{centering}
\end{table}
